Age of Information Under Frame Slotted ALOHA-Based Status Updating Protocol

We propose a frame slotted ALOHA (FSA)-based protocol for a random access network where sources transmit status updates to their intended destinations. We evaluate the effect of such a protocol on the network's timeliness performance using the Age of Information (AoI) metric. Specifically, we leverage tools from stochastic geometry to model the spatial positions of the source-destination pairs and capture the entanglement amongst the nodes' spatial-temporal attributes through the interference they caused to each other. We derive analytical expressions for the average and variance of AoI over a typical transmission link in Poisson bipolar and cellular networks, respectively. Our analysis shows that in densely deployed networks, the FSA-based status updating protocol can significantly decrease the average AoI and in addition, stabilizes the age performance by substantially reducing the variance of AoI. Furthermore, under the same updating frequency, converting a slotted ALOHA protocol into an FSA-based one always leads to a reduction in the average AoI. Moreover, implementing FSA in conjunction with power control can further benefit the AoI performance, although the particular values of framesize and power control factor must be adequately tuned to achieve the optimal gain.

==> AoI under Frame Slotted ALOHA/SupportDocuments/aconym.tex <==

%----- V2 ------
\acrodef{CCDF}{complementary cumulative distribution function}
\acrodef{CF}{characteristic function}
%\acrodef{PPP}{Poisson point process}
\acrodef{PPP}{Poisson point processe}
%----- V1 ------
\acrodef{RV}{random variable}
%\acrodef{rv}{random variable}
\acrodef{i.i.d.}{independent and identically distributed}
\acrodef{PDF}{probability distribution function}
%\acrodef{pdf}{probability distribution function}
\acrodef{CDF}{cumulative distribution function}
\acrodef{ch.f.}{characteristic function}
\acrodef{AWGN}{additive white Gaussian noise}
\acrodef{SNR}{signal-to-noise ratio}
\acrodef{LRT}{likelihood ratio test}
\acrodef{DRT}{distance ratio test}
\acrodef{GLRT}{generalized likelihood ratio test}
\acrodef{CRLB}{Cram\'{e}r-Rao lower bound}
\acrodef{CRB}{Cram\'{e}r-Rao bound}
\acrodef{ZZLB}{Ziv-Zakai lower bound}
\acrodef{ZZB}{Ziv-Zakai bound}
\acrodef{LOS}{line-of-sight}
\acrodef{ToF}{time-of-flight}
\acrodef{NLOS}{non-line-of-sight}
\acrodef{GDOP}{geometric dilution of precision}
\acrodef{GPS}{Global Positioning System}
\acrodef{FIM}{Fisher information matrix}
\acrodef{PEB}{position error bound}
\acrodef{SPEB}{squared position error bound}
\acrodef{TOA}{time-of-arrival}
\acrodef{TOF}{time-of-flight}
\acrodef{WSN}{wireless sensor network}
\acrodef{MAC}{medium access control}
\acrodef{RSS}{received signal strength}
\acrodef{WAF}{wall attenuation factor}
\acrodef{TDOA}{time difference-of-arrival}
\acrodef{RF}{radiofrequency}
\acrodef{RTT}{round-trip time}
\acrodef{AOA}{angle-of-arrival}
\acrodef{MF}{matched filter}
\acrodef{ED}{energy detector}
\acrodef{ML}{maximum likelihood}
\acrodef{MSE}{mean-square error}
\acrodef{RMSE}{root-mean-square error}
\acrodef{LEO}{localization error outage}
\acrodef{ppm}{part-per-million}
\acrodef{ACK}{acknowledge}
\acrodef{UWB}{Ultrawide bandwidth}
\acrodef{TNR}{threshold-to-noise ratio}
\acrodef{LS}{least squares}
\acrodef{IR-UWB}{impulse radio UWB}
\acrodef{FCC}{Federal Communications Commission}
\acrodef{TH}{time-hopping}
\acrodef{PPM}{pulse position modulation}
\acrodef{MUI}{multi-user interference}
\acrodef{PDP}{power delay profile}
\acrodef{BPZF}{band-pass zonal filter}
\acrodef{SIR}{signal-to-interference ratio}
\acrodef{SINR}{signal-to-interference-plus-noise ratio}
\acrodef{RFID}{radio frequency identification}
\acrodef{WPAN}{wireless personal area network}
\acrodef{WWB}{Weiss-Weinstein bound}
\acrodef{DP}{direct path}
\acrodef{MF}{matched filter}
\acrodef{MMSE}{minimum-mean-square-error}
\acrodef{SBS}{serial backward search}
\acrodef{SBSMC}{serial backward search for multiple clusters}
\acrodef{NBI}{narrowband interference}
\acrodef{WBI}{wideband interference}
\acrodef{INR}{interference-to-noise ratio}
\acrodef{CR}{channel response}
\acrodef{CIR}{channel impulse response}
\acrodef{CR}{channel  response}
%\acrodef{LRT}{likelihood ratio test}
\acrodef{RADAR}{radar}
\acrodef{MUR}{Multistatic radar}
\acrodef{JBSF}{jump back and search forward}
\acrodef{HDSA}{high-definition situation-aware}
\acrodef{RRC}{root raised cosine}
\acrodef{ST}{simple thresholding}
\acrodef{BTB}{Bellini-Tartara bound}
\acrodef{P-Max}{$P$-Max}  %suggestion, use with \acl{P-Max}
\acrodef{MIMO}{multiple-input multiple-output}
\acrodef{MAP}{maximum a posteriori}
\acrodef{FG}{factor graph}
\acrodef{OP}{outage probability}
\acrodef{WED}{wall extra delay}
\acrodef{RMS}{root mean square}
\acrodef{SPAWN}{sum-product algorithm over a wireless network}
\acrodef{MDD}{minimum distance distribution}
\acrodef{MAP}{maximum a posteriori probability}
\acrodef{SAP}{small cell access point}
\acrodef{UE}{user equipment}
\acrodef{MBS}{macro cell base station}
\acrodef{UER}{\ac{UE} Relay}
\acrodef{D2D}{device-to-device}
\acrodef{MBS}{macro base station}
\acrodef{CSI}{channel state information}
\acrodef{OGR}{outage guard region}
\acrodef{FUR}{feasible UER region}
\acrodef{EHR}{energy harvesting region}
\acrodef{EH}{energy harvesting}
\acrodef{D2D-EHSN}{D2D communication provided \ac{EH} small cell network}
\acrodef{D2D-EHHN}{D2D communication provided \ac{EH} heterogeneous network}
\acrodef{3GPP}{3rd Generation Partnership Project}
\acrodef{BS}{base station}
\acrodef{DF}{decode and forward}
\acrodef{CCDF}{complementary cumulative distribution function}
\acrodef{ZF}{zero forcing}
\acrodef{RZF}{regularized zero forcing}
\acrodef{WLLN}{weak law of large number}
\acrodef{SLLN}{strong law of large numbers}
\acrodef{TDD}{Time-division duplex}
\acrodef{EE}{energy efficiency} 
\acrodef{HetNet}{heterogeneous network} 
\acrodef{SCP}{Single Cell Processing}
\acrodef{CBF}{Coordinated Beamforming}

==> AoI under Frame Slotted ALOHA/SupportDocuments/defmetric.tex <==
% put your latex definitions here.
% For example: \newcommand{\samplesize}{n}
%---------------------%
% Package          %
%---------------------%
\usepackage{color}
%\usepackage[usenames]{color}
\usepackage{dsfont}
\usepackage{bbm}

%---------------------%
% References          %
%---------------------%
%\newcommand{\fig}[1]{Fig.~\ref{#1}}
%\newcommand{\sect}[1]{Sec.~\ref{#1}}
%\newcommand{\apd}[1]{Appendix~\ref{#1}}
%\newcommand{\eq}[1]{(\ref{#1})}

%---------------------%
% Symbols             %
%---------------------%
\newcommand{\ChG}[1]{ \left| \RV{h}_{#1} \right|^2}
%\newcommand{\CCDF}[2]{{\bar{F}_{#1}}\left({#2}\right)}
%\newcommand{\IndFb}[1]{\mathds{1}\left(#1 \right)}
\newcommand{\IndFb}[1]{\mathbbm{1}\left(#1 \right)}
\newcommand{\IndF}[2]{\mathbbm{1}_{#1}\left(#2 \right)}
\newcommand{\xs}[1]{x_{\text{s}_{#1}}}
\newcommand{\xu}[1]{x_{\text{u}_{#1}}}
\newcommand{\s}[1]{\mathbf{s}_{#1}}
\newcommand{\ws}[1]{\mathbf{w}_{\text{s}_{#1}}}
\newcommand{\wu}[1]{\mathbf{w}_{\text{u}_{#1}}}
%====================================
\def\x{\RV{X}}
\def\y{\RV{Y}}
\def\NB{N_{\text{b}}}
\def\NS{N_{\text{s}}}
\def\PMT{P_{\mathrm{mt}}}
\def\PST{P_{\mathrm{st}}}
\def\PUT{P_{\mathrm{ut}}}
\def\PMD{P_{\mathrm{md}}}
\def\PSD{P_{\mathrm{sd}}}
\def\PUD{P_{\mathrm{ud}}}
\def\PM{P_{\mathrm{mt}}}
\def\PB{P_{\mathrm{bt}}}
\def\PS{P_{\mathrm{st}}}
\def\PU{P_{\mathrm{ut}}}
%\def\KM{K_\mathrm m}
\def\KM{K}
\def\KS{K_\mathrm s}
\def\KB{K_\mathrm b}
\def\MM{M_\mathrm m}
\def\MS{M_\mathrm s}
%\def\NM{N_\mathrm m}
\def\NM{N}
\def\NS{N_\mathrm s}
\def\LM{\lambda}
\def\LB{\lambda_{\mathrm{b}}}
\def\LS{\lambda_{\mathrm{s}}}
\def\LU{\lambda_{\mathrm{u}}}
\def\SNRB{\rho_{\mathrm{b}}}
\def\SNRS{\rho_{\mathrm{s}}}
\def\SNRU{\rho_{\mathrm{u}}}
\def\hH{\hat{\mathbf{H}}}
\def\hh{\hat{\mathbf{h}}}
\def\PDM{\tau_{\mathrm{m}}}
\def\PDS{\tau_{\mathrm{s}}}
\def\PDMS{\tau_{\mathrm{b}}}
\def\TS{\theta_{\mathrm{s}}}
%---------------------%
% Notes             %
%---------------------%
\newcommand{\mynote}[1]{%
\noindent \textcolor{blue}{\framebox{$\triangleright$ %
{\small\textsf{#1}} $\triangleleft$}}}

%---------------------%
% References          %
%---------------------%

\renewcommand{\IEEEQED}{\IEEEQEDopen}

\renewcommand{\sfdefault}{cmbr}
\DeclareMathAlphabet{\mathsf}{OML}{cmbr}{m}{it}
\newcommand{\red}[1]{{\textcolor[rgb]{1,0,0}{#1}}}


\newtheorem{definition}{\bf Definition}
\newtheorem{theorem}{\bf Theorem}
\newtheorem{lemma}{\bf Lemma}
\newtheorem{corollary}{\bf Corollary}
\newtheorem{proposition}{\bf Proposition}
\newtheorem{example}{\bf Example}
\newtheorem{remark}{\bf Remark}
\newtheorem{property}{\bf Property}
%\newtheorem{algorithm}{\bf Algorithm}
\newtheorem{assumption}{\bf Assumption}

\DeclareMathOperator{\vecOp}{\mathrm{vec}}
\DeclareMathOperator{\tr}{\mathrm{tr}}
\DeclareMathOperator{\E}{\mathds{E}}
\DeclareMathOperator{\var}{\mathds{V}\mathrm{ar}}
\DeclareMathOperator{\prob}{\mathds{P}}
% \DeclareMathOperator{\re}{\mathfrak{Re}}
\DeclareMathOperator{\im}{\mathfrak{Im}}

\newcommand{\N}{\mathbbmss{N}}
\newcommand{\R}{\mathbbmss{R}}
% \newcommand{\C}{\mathbbmss{C}}
\newcommand{\Z}{\mathbbmss{Z}}
%\newcommand{\B}[1]{\mathbf{#1}}
\newcommand{\B}[1]{\pmb{#1}}

\newcommand{\RV}[1]{\mathsf{#1}}
%
\newcommand{\PX}[1] {{\mathbb{P}}\left\{{#1}\right\}}
\newcommand{\EX}[1] {{\mathbb{E}}\left\{{#1}\right\}}
%\newcommand{\EX}[1]{\E\left\{{#1}\right\}}
\newcommand{\EXs}[2] {{\mathbb{E}}_{{#1}}\!\!\left\{{#2}\right\}}
%\newcommand{\EXs}[2]{\E_{{#1}}\left\{{#2}\right\}}
\newcommand{\PDF}[2]{p_{{#1}}\left({#2}\right)}
\newcommand{\CDF}[2]{F_{{#1}}\left({#2}\right)}
\newcommand{\CCDF}[2]{{\bar{F}_{#1}}\left({#2}\right)}
\newcommand{\MGF}[2]{\phi_{#1}\left({#2}\right)}
\newcommand{\Var}[1]{\var\left\{{#1}\right\}}
\newcommand{\Prob}[1]{\prob\left\{{#1}\right\}}
\newcommand{\Bern}[1]{\textsf{Bern}\left({#1}\right)}
\newcommand{\Binom}[2]{\textsf{Binom}\left({#1},{#2}\right)}
\newcommand{\Erl}[2]{\textsf{Erl}\left(#1,#2\right)}
\newcommand{\Exp}[1]{\textsf{Exp}\left(#1\right)}
% \newcommand{\RE}[1]{\re\left\{{#1}\right\}}
\newcommand{\Imag}[1]{\im\left\{{#1}\right\}}


\newcommand{\RG}[2]{\mathcal{N}\left({#1},{#2}\right)}
\newcommand{\CG}[2]{\mathcal{CN}\left({#1},{#2}\right)}
\newcommand{\RGV}[3]{\mathcal{N}_{{#1}}\left({#2},{#3}\right)}
\newcommand{\CGV}[3]{\tilde{\mathcal{N}}_{{#1}}\left({#2},{#3}\right)}
\newcommand{\CGM}[5]{\tilde{\mathcal{N}}_{{#1},{#2}}\left({#3},{#4},{#5}\right)}
\newcommand{\CWM}[3]{\tilde{\mathcal{W}}_{#1}\left({#2},{#3}\right)}

\newcommand{\GF}[1]{\Gamma\left(#1\right)}

\newcommand{\sNorm}[1]{\left|{#1}\right|}
\newcommand{\vNorm}[1]{\left\|{#1}\right\|}

%--------------------------------------------------------------%
% List: Using description, enumerate, itemize       %
%--------------------------------------------------------------%

\newcommand{\bd}{\begin{description}}
\newcommand{\ed}{\end{description}}
\newcommand{\be}{\begin{enumerate}}
\newcommand{\ee}{\end{enumerate}}
\newcommand{\bi}{\begin{itemize}}
\newcommand{\ei}{\end{itemize}}
\newcommand{\bl}{\begin{list}}
\newcommand{\el}{\end{list}}
\newcommand{\bt}{\begin{tabbing}}
\newcommand{\et}{\end{tabbing}}

